SeqAfford: Sequential 3D Affordance Reasoning via Multimodal Large Language Model

3D affordance segmentation aims to link human instructions to touchable regions of 3D objects for embodied manipulations. Existing efforts typically adhere to single-object, single-affordance paradigms, where each affordance type or explicit instruction strictly corresponds to a specific affordance region and are unable to handle long-horizon tasks. Such a paradigm cannot actively reason about complex user intentions that often imply sequential affordances. In this paper, we introduce the Sequential 3D Affordance Reasoning task, which extends the traditional paradigm by reasoning from cumbersome user intentions and then decomposing them into a series of segmentation maps. Toward this, we construct the first instruction-based affordance segmentation benchmark that includes reasoning over both single and sequential affordances, comprising 180K instruction-point cloud pairs. Based on the benchmark, we propose our model, SeqAfford, to unlock the 3D multi-modal large language model with additional affordance segmentation abilities, which ensures reasoning with world knowledge and fine-grained affordance grounding in a cohesive framework. We further introduce a multi-granular language-point integration module to endow 3D dense prediction. Extensive experimental evaluations show that our model excels over well-established methods and exhibits open-world generalization with sequential reasoning abilities.

==> sup.tex <==
\clearpage
\setcounter{page}{1}
% \maketitlesupplementary
\onecolumn
\begin{center}
{ \linespread{1.5} \selectfont
\textbf{\Large Global and Local Prompts Cooperation via Optimal Transport \\
for Federated Learning} \\
}
\Large Supplementary Materials
\end{center}
\appendix
\setcounter{table}{0}   %从0开始编号，显示出来表会A1开始编号
\setcounter{figure}{0}

%定义编号格式，在数字序号前加字符“A"
\renewcommand{\thetable}{A\arabic{table}}
\renewcommand{\thefigure}{A\arabic{figure}}
\makeatletter

% This section contains supplementary material that provides additional details for the main paper and further experimental analysis. This section follows the contents in the following order:

\startcontents[appendix]
\printcontents[appendix]{l}{1}{\section*{Supplementary organization:}\setcounter{tocdepth}{2}}
% \tableofcontents
% \DoToC
% \localtableofcontents

% \renewcommand{\labelitemii}{\textbullet}
% \begin{enumerate}[label=\Alph*]
%     \item Method Details \newline
%         A.1 Training Process \newline
%         A.2 Efficient scaling Dykstra’s Algorithm
%     \item Experimental Details \newline
%         B.1 Details of Dataset Setup \newline
%         B.2 Implementation Details
%     \item Additional Experiments Results
%     \item Visualization
%     \item Generalization Bound \newline
%         E.1 Key Lemmas \newline
%         E.2 Proof of Theorem 1
% \end{enumerate}

% \item Method Details (Appendix A)
% \item Experimental Details (Appendix B)
%     \begin{itemize}
%     \item Details of Dataset Setup
%     \item Implementation Details
%     \end{itemize}
% \end{itemize}

% \newpage



